Query2Label: A Simple Transformer Way to Multi-Label Classification

This paper presents a simple and effective approach to solving the multi-label classification problem. The proposed approach leverages Transformer decoders to query the existence of a class label. The use of Transformer is rooted in the need of extracting local discriminative features adaptively for different labels, which is a strongly desired property due to the existence of multiple objects in one image. The built-in cross-attention module in the Transformer decoder offers an effective way to use label embeddings as queries to probe and pool class-related features from a feature map computed by a vision backbone for subsequent binary classifications. Compared with prior works, the new framework is simple, using standard Transformers and vision backbones, and effective, consistently outperforming all previous works on five multi-label classification data sets, including MS-COCO, PASCAL VOC, NUS-WIDE, and Visual Genome. Particularly, we establish $91.3\%$ mAP on MS-COCO. We hope its compact structure, simple implementation, and superior performance serve as a strong baseline for multi-label classification tasks and future studies. The code will be available soon at https://github.com/SlongLiu/query2labels.

==> tables/ablation.tex <==
\begin{table}[hbt!]
\centering

\begin{tabular}{c|c|c|c} 
\hline
Method & Backbone &  GMac & mAP   \\ 
\hline
Baseline & ResNet101 & 31.39 & 81.6 \\
Q2L-1d & ResNet101 & 33.18 & 83.2 \\
Q2L-2d & ResNet101 & 34.13  & 83.4 \\
Q2L-1e-1d & ResNet101 & 35.50 & 83.5 \\
Q2L-1e-2d & ResNet101 & 36.45 & 83.7 \\
\hline
Baseline & TResNetL & 43.52 & 85.1 \\
Q2L-1d & TResNetL & 45.62(+4.8\%) & 86.4 \\
Q2L-2d & TResNetL & 46.57(+7.0\%) & 86.6 \\
Q2L-1e-1d & TResNetL & 47.94(+10.2\%) & 86.4 \\
Q2L-1e-2d & TResNetL & 48.89(+12.3\%) & 86.9 \\
\hline
\end{tabular}

\caption{Computational complexity comparison between Query2Label and prior state-of-the-art baselines.}
\label{Table:ablation}

\end{table}

==> tables/ablation_single.tex <==
\begin{table}[hbt!]
\centering

\begin{tabular}{c|c|c|c} 
\hline
Method  & GMac & Prameters & mAP   \\ 
\hline
Baseline~\cite{ridnik2020tresnet} (TResNetL) & \multirow{2}{*}{43.52} & \multirow{2}{*}{53.75 M} & 85.1 \\
ASL~\cite{benbaruch2020asymmetric}(TResNetL) &  &  & 86.6 \\
\hline
% Baseline~\cite{ridnik2020tresnet} (TResNetL) & {43.52} & {53.75 M} & 85.1 \\
Ours(TResNetL+Q2L-xs) & \textbf{43.23} & \textbf{35.79} M & \textbf{86.7} \\
\hline
\end{tabular}
\vspace{0.1cm}
\caption{Computational complexity comparison between Query2Label and prior state-of-the-art baselines. Q2L-xs is a lite version of Q2L. Refer to the text for more details about Q2L-xs.
% To reduce the model size and computational complexity, we use only $1$ Transformer decoder and remove the self-attention module in the decoder, the 16th Bottleneck in layer 3 of the backbone, and the input projection layer in Q2L-xs.
}
\label{Table:abla_single}
% \shilong{There are many results about TResNetL: in original paper: 86.4(Baseline); in ASL paper: 83.1(Baseline), 85.1(focal), 86.6(ASL); in my experiments: 85.1(Baseline+different $\gamma$ for pos and neg samples).}
\vspace{-0.5cm}
\end{table}

==> tables/coco_maintext_v2.tex <==
\begin{table*}[hbt!]
\setlength{\tabcolsep}{5pt}
\centering
\begin{tabular}{c|c|c|c|c|c|c|c} 
\hline
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & 
\multicolumn{1}{c|}{\multirow{2}{*}{Backbone}} & 
\multicolumn{1}{c|}{\multirow{2}{*}{Resolution}} & 
\multicolumn{1}{c|}{\multirow{2}{*}{mAP}} & 
\multicolumn{2}{c|}{All}  & \multicolumn{2}{c}{Top 3} \\ 
\cline{5-8}
\multicolumn{1}{l|}{} &&&&CF1 &  
\multicolumn{1}{l|}{OF1} & CF1 & OF1 \\ 
\hline
\hline
CADM~\cite{8784938} & ResNet101 & 448$\times$448 & 82.3 &  77.0 &  79.6 & 73.5 & 76.0 \\
ML-GCN~\cite{ML-GCN_CVPR_2019} & ResNet101 & 448$\times$448 & 83.0 & 78.0  & 80.3  & 74.2  & 76.3 \\
KSSNet~\cite{liu2018multi} & ResNet101 & 448$\times$448 & 83.7 &  77.2 &  81.5  & - & - \\
MS-CMA~\cite{you2020cross} & ResNet101 & 448$\times$448 & 83.8 &  78.4 & 81.0  & 74.3   & 77.2  \\
MCAR~\cite{gao2020multi} & ResNet101 & 448$\times$448 & 83.8 & 78.0& 80.3   & {75.1}    & 76.7  \\ 
SSGRL~\cite{chen2019learning} & ResNet101 & 576$\times$576  & 83.8  & 76.8  & 79.7  & 72.7  & 76.2  \\ 
C-Trans~\cite{lanchantin2020general} & ResNet101 & 576$\times$576  & 85.1  & 79.9  & 81.7  & 76.0  & 77.6  \\ 
ADD-GCN~\cite{ye2020attention} & ResNet101 & 576$\times$576 & 85.2  & 80.1  & 82.0  & 75.8   & 77.9  \\ 
\hline
Q2L-R101(Ours) & ResNet101 & 448$\times$448 &  {84.9} &  {81.6} &  {83.1}  &  {77.0} &   {78.5}  \\
Q2L-R101(Ours) & ResNet101 & 576$\times$576 &  \textbf{86.5} &  \textbf{81.6} &  \textbf{83.1}  &  \textbf{77.0} &   \textbf{78.5}  \\
\hline
\hline
ASL~\cite{benbaruch2020asymmetric} & TResNetL & 448$\times$448 & {86.6} & {81.4} &  {81.8}   & {75.1}  & {77.4}    \\
TResNetL~\cite{ridnik2021imagenet21k} & TResNetL(22k) & 448$\times$448 & {88.4} & - &  -  & -  & -   \\
\hline
Q2L-TResL(Ours) & TResNetL & 448$\times$448 &  {{87.3}} &  {81.6} &  {83.1}  &  {77.0} &   {78.5}  \\
Q2L-TResL(Ours) & TResNetL(22k) & 448$\times$448 &  {\textbf{89.2}} &  \textbf{81.6} &  \textbf{83.1} &  \textbf{77.0} &  \textbf{78.5}  \\
\hline
\hline
MlTr-l~\cite{cheng2021mltr} & MLTr-l(22k) & 384$\times$384 & {88.5} & {83.3} &  {84.9}   & -  & -  \\
Swin-L~\cite{liu2021swin} & Swin-L(22k) & 384$\times$384 & 89.6 & - & - & - & - \\
CvT-w24~\cite{wu2021cvt} & CvT-w24(22k) & 384$\times$384 & 90.5 & - & - & - & - \\
\hline
Q2L-SwinL(Ours) & Swin-L(22k) & 384$\times$384 &  {90.5} &  - &  - & - & -\\
Q2L-CvT(Ours) & CvT-w24(22k) & 384$\times$384 &  {\textbf{91.3}} &  - &  - & - & -\\
\hline
\hline
\end{tabular}
\vspace{0.3cm}
\caption{Comparison of our method with known state-of-the-art models on MS-COCO at medium input resolution. The backbones noted with 22k are pretrained on ImageNet-22k dataset.
Among them, mAP, OF1, and CF1 are the primary metrics (shaded in the table) as the others may be affected by the chosen threshold largely. All metrics are in \%.}
\label{Table:coco}
\end{table*}

==> tables/coco_meduim_resolution.tex <==
\begin{table*}[hbt!]
\setlength{\tabcolsep}{5pt}
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & 
\multicolumn{1}{c|}{\multirow{2}{*}{mAP}} & 
\multicolumn{6}{c|}{All}  & \multicolumn{6}{c}{Top 3} \\ 
\cline{3-14}
\multicolumn{1}{l|}{} &&CP & CR & CF1 & OP & OR & 
\multicolumn{1}{l|}{OF1} & CP & CR & CF1 & OP & OR & OF1 \\ 
% \cline{2-14}
% \multicolumn{1}{l|}{} & mAP & CP & CR & CF1 & OP & OR & \multicolumn{1}{l|}{OF1} & CP & CR & CF1 & OP & OR & OF1 \\ 

\hline
CADM~\cite{8784938} & 82.3 & 82.5 & 72.2 & 77.0 & 84.0 & 75.6 & 79.6 & 87.1 & 63.6 & 73.5 & 89.4 & 66.0 & 76.0 \\
ML-GCN~\cite{ML-GCN_CVPR_2019} & 83.0 & 85.1 & 72.0 & 78.0 & 85.8 & 75.4 & 80.3 & 87.2 & 64.6 & 74.2 & 89.1 & 66.7 & 76.3 \\
KSSNet~\cite{liu2018multi} & 83.7 & 84.6 & 73.2 & 77.2 & 87.8 & 76.2 & 81.5 & - & - & - & - & - & - \\
MS-CMA~\cite{you2020cross} & 83.8 & 82.9 & 74.4 & 78.4 & 84.4 & 77.9 & 81.0 & 86.7 & 64.9  & 74.3   & 90.9  & {67.2}  & 77.2  \\
MCAR~\cite{gao2020multi} & 83.8 & 85.0 & 72.1 & 78.0 & 88.0 & 73.9 & 80.3  & 88.1  & {65.5}  & {75.1}   & 91.0  & 66.3  & 76.7  \\ 
ADD-GCN~\cite{ye2020attention} (512) & 85.2 & 84.7 & 75.9 & 80.1 & 84.9 & \textbf{79.4} & 82.0 & 88.8  & \textbf{66.2}  & 75.8 & 90.3  & \textbf{68.5}  & 77.9  \\ 
SSGRL~\cite{chen2019learning} (576) & 83.8 & \textbf{89.9} & 68.5 & 76.8 & \textbf{91.3} & 70.8 & 79.7 & \textbf{91.9}  & 62.5 & 72.7 & 93.8 & 64.1 & 76.2  \\ 
ASL (TResNetL)~\cite{benbaruch2020asymmetric} & {86.6} & {87.2} & {76.4} & {81.4} & {88.2} & {79.2} & {81.8}  & {91.8}  & 63.4  & {75.1} & {92.9} & 66.4 & {77.4}    \\
\hline
Ours (ResNet101+Q2L) &  \textbf{84.6} & {87.6} & \textbf{76.5} & \gray \textbf{81.6} & {88.4} & {78.5} & \gray \textbf{83.1} & 
\textbf{91.9} & \textbf{66.2} & \gray \textbf{77.0} & \textbf{93.5} & {67.6} & \gray \textbf{78.5}  \\
Ours (TResNetL+Q2L) & \gray {\textbf{87.3}} & {87.6} & \textbf{76.5} & \gray \textbf{81.6} & {88.4} & {78.5} & \gray \textbf{83.1} & 
\textbf{91.9} & \textbf{66.2} & \gray \textbf{77.0} & \textbf{93.5} & {67.6} & \gray \textbf{78.5}  \\
Ours (TResNetL+Q2L+ImageNet22k) & \gray {\textbf{89.2}} & {87.6} & \textbf{76.5} & \gray \textbf{81.6} & {88.4} & {78.5} & \gray \textbf{83.1} & 
\textbf{91.9} & \textbf{66.2} & \gray \textbf{77.0} & \textbf{93.5} & {67.6} & \gray \textbf{78.5}  \\
\hline
\end{tabular}
\vspace{0.3cm}
\caption{Comparison of our method with known state-of-the-art models on MS-COCO at medium input resolution. All results are reported at resolution 448 except for ADD-GCN and SSGRL, whose resolutions are noted in parentheses. Among them, mAP, OF1, and CF1 are the primary metrics (shaded in the table) as the others may be affected by the chosen threshold largely. All metrics are in \%.}
\label{Table:coco}
\end{table*}

==> tables/multihead_table.tex <==
\begin{table}[hbt!]
\centering

\begin{tabular}{c|c|c} 
\hline
Method & nheads & mAP   \\ 
\hline
Q2L-1e-2d & 1 & 86.6 \\
Q2L-1e-2d & 2 & 86.6 \\
Q2L-1e-2d & 4 & 86.9 \\
Q2L-1e-2d & 8 & 87.0 \\
Q2L-1e-2d & 16 & 87.0 \\
Q2L-1e-2d & 32 & 86.9 \\
Q2L-1e-2d & 64 & 86.9 \\
Q2L-1e-2d & 128 & 86.4 \\
Q2L-1e-2d & 304 & 86.5 \\
\hline
\end{tabular}

\caption{Impact of the number of heads.}
\label{Table:multihead}

\end{table}

==> tables/voc2007.tex <==
\begin{table*}[t]
	\centering
	
	
	\resizebox{\textwidth}{!}{
		\begin{tabular}{|@{\,}c@{\,}||@{\,}c@{\,}|| *{20}{@{\,}c@{\,}}||@{\,}c@{\,}|}
			\hline
			Methods  &Backbone &aero &bike &bird &boat &bottle &bus &car &cat &chair &cow &table &dog &horse &mbike &person &plant &sheep &sofa &train &tv &mAP\\
			\hline
% 			\hline
			CNN-RNN~\cite{wang2016cnn} &VGG16                &96.7 &83.1 &94.2 &92.8 &61.2 &82.1 &89.1 &94.2 &64.2 &83.6 &70.0 &92.4  &91.7 &84.2 &93.7 &59.8 &93.2 &75.3 &\textbf{99.7} &78.6 &84.0\\
			VGG+SVM~\cite{simonyan2015very} &~VGG16\&19~  &98.9 &95.0 &96.8 &95.4 &69.7 &90.4 &93.5 &96.0 &74.2 &86.6 &87.8 &96.0 &96.3 &93.1 &97.2 &70.0 &92.1 &80.3 &98.1 &87.0 &89.7\\
			Fev+Lv~\cite{yang2016exploit} &VGG16                  &97.9 &97.0 &96.6 &94.6 &73.6 &93.9 &96.5 &95.5 &73.7 &90.3 &82.8 &95.4 &97.7 &95.9 &98.6 &77.6 &88.7 &78.0 &98.3 &89.0 &90.6\\
			HCP~\cite{wei2015hcp} &VGG16                             &98.6 &97.1 &98.0 &95.6 &75.3 &94.7 &95.8 &97.3 &73.1 &90.2 &80.0 &97.3 &96.1 &94.9 &96.3 &78.3 &94.7 &76.2 &97.9 &91.5 &90.9\\
            RDAL~\cite{wang2017multi}  &VGG16        &98.6 &97.4 &96.3 &96.2 &75.2 &92.4 &96.5 &97.1 &76.5 &92.0 &87.7 &96.8 &97.5 &93.8 &98.5 &81.6 &93.7 &82.8 &98.6 &89.3 &91.9\\
            RARL~\cite{chen2018recurrent} &VGG16  &98.6 &97.1 &97.1 &95.5 &75.6 &92.8 &96.8 &97.3 &78.3 &92.2 &87.6 &96.9 &96.5 &93.6 &98.5 &81.6 &93.1 &83.2 &98.5 &89.3 &92.0\\
            % SSGRL*~\cite{chen2019learning} &ResNet-101                 &99.5 &97.1 &97.6 &97.8 &82.6 &94.8 &96.7 &98.1 &78.0 &\textbf{97.0} &85.6 &97.8 &98.3 &96.4 &98.1 &\textbf{84.9} &96.5 &79.8 &98.4 &92.8 &93.4\\
            % \hline                                                         
            % Baseline &ResNet-101                                              &99.0&97.9&97.2&97.6&80.2&93.6&96.0&98.0&81.8&92.0&84.6&97.5&97.2&95.3&97.9&81.8&94.6&84.1&98.2&93.6 &92.9\\
            SSGRL~\cite{chen2019learning} (576) &ResNet-101  &99.7 & 98.4  & 98.0  & 97.6  & 85.7 &  96.2 &  98.2 &  98.8 &  82.0 &  98.1  & 89.7 &  98.8  & 98.7  & 97.0  & 99.0  & 86.9  & 98.1  & 85.8  & 99.0 &  93.7 &  95.0\\
            ADD-GCN~\cite{ye2020attention} (512) &ResNet-101  & 99.8  &  99.0  &  98.4  &  99.0  &  86.7  &  98.1  &  98.5  &  98.3  &  85.8  &  98.3  &  88.9  &  98.8  &  99.0  &  97.4  &  99.2  &  88.3  &  98.7  &  90.7  &  99.5  &  97.0  &  96.0 \\
            MCAR~\cite{gao2020learning} &ResNet-101&	\textbf{99.7} &\textbf{99.0}& 98.5&\textbf{98.2}&\textbf{85.4}&\textbf{96.9}&\textbf{97.4}&\textbf{98.9}&\textbf{83.7}& 95.5&\textbf{88.8}&\textbf{99.1}& 98.2& 95.1&\textbf{99.1}& 84.8&\textbf{97.1}&\textbf{87.8}& 98.3&\textbf{94.8} &{94.8} \\ 	
            ASL~\cite{benbaruch2020asymmetric} & TResNetL &-& & & & & & & &-& -&-& - & - & - & - & - &- & - & - & - &{95.8} \\ 
            \hline
            Ours & TResNetL &-& & & & & & & &-& -&-& - & - & - & - & - &- & - & - & - &\textbf{96.1} \\ 
            \hline
	\end{tabular}}

	\caption{Comparisons of our method with previous state-of-the-art methods on the PASCAL VOC 2007. The evaluation metrics are AP and mAP in $\%$.  
	$*$ indicates methods using a larger input size. \leizhang{where are the stars?}}
    \label{table:voc07}
\end{table*} 

==> tables/voc2012.tex <==
\begin{table*}[t]
	\centering
		
		\footnotesize
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|@{\,}c@{\,}||@{\,}c@{\,}|| *{20}{@{\,}c@{\,}}||@{\,}c@{\,}|}
				\hline
				Methods &Backbone &aero &bike &bird &boat &bottle &bus &car &cat &chair &cow &table &dog &horse &mbike &person &plant &sheep &sofa &train &tv &mAP\\
				\hline
				VGG+SVM~\cite{simonyan2015very} &VGG16\&19                  &99.0 &89.1 &96.0 &94.1 &74.1 &92.2 &85.3 &97.9 &79.9 &92.0 &83.7 &97.5 &96.5 &94.7 &97.1 &63.7 &93.6 &75.2 &97.4 &87.8 &89.3\\			        
			        	Fev+Lv~\cite{yang2016exploit} &VGG16                         &98.4 &92.8 &93.4 &90.7 &74.9 &93.2 &90.2 &96.1 &78.2 &89.8 &80.6 &95.7 &96.1 &95.3 &97.5 &73.1 &91.2 &75.4 &97.0 &88.2 &89.4\\
				HCP~\cite{wei2015hcp}                                                    &VGG16 &99.1 &92.8 &97.4 &94.4 &79.9 &93.6 &89.8 &98.2 &78.2 &94.9 &79.8 &97.8 &97.0 &93.8 &96.4 &74.3 &94.7 &71.9 &96.7 &88.6 &90.5\\
				SSGRL*~\cite{chen2019learning} &ResNet-101                       &99.5 &95.1 &97.4 &96.4 &85.8 &94.5 &93.7 &{98.9} &86.7 &96.3 &84.6 &{98.9} &{98.6} &96.2 &98.7 &82.2 &{98.2} &{84.2}&98.1 &93.5 &93.9\\
				MCAR~\cite{gao2020learning} &ResNet-101                                                       &{99.6} &{97.1}&{98.3}&{96.6}&{87.0}&{95.5}&{94.4}&98.8&{87.0}&{96.9}&{85.0}&98.7&98.3&{97.3}&{99.0}&{83.8}&96.8&83.7&{98.3}&93.5  &{94.3}\\
				SSGRL~\cite{chen2019learning}(576) &ResNet-101 & 99.7 &  96.1  & 97.7 &  96.5 &  86.9  & 95.8 &  95.0 &  98.9  & 88.3  & 97.6 &  87.4 &  99.1  & 99.2 &  97.3  & 99.0 &  84.8  & 98.3  & 85.8 &  99.2 &  94.1  & 94.8 \\
				ADD-GCN~\cite{ye2020attention}(512) &ResNet-101 & 99.8 &  97.1 &  98.6 &  96.8 &  89.4 &  97.1 &  96.5 &  99.3 &  89.0  & 97.7  & 87.5 &  99.2  & 99.1  & 97.7 &  99.1 &  86.3 &  98.8 &  87.0 &  99.3 &  95.4  & 95.5 \\
				\hline
				Ours & TResNetL                                                      &\textbf{99.9} &\textbf{98.2}&\textbf{99.3}&\textbf{98.1}&\textbf{90.4}&\textbf{97.7}&\textbf{97.4}&\textbf{99.4}&\textbf{92.7}&\textbf{98.7}&\textbf{89.9}&\textbf{99.4}&\textbf{99.5}&\textbf{99.0}&\textbf{99.4}&\textbf{88.4}&\textbf{98.8}&\textbf{89.3}&\textbf{99.6}&\textbf{96.8}  &\textbf{96.6}\\
				\hline
	\end{tabular}}
	\caption{Comparisons of AP and mAP in $\%$ of our model and state-of-the-art methods on the PASCAL VOC 2012. $*$ indicates methods using larger input size.}
	\label{table:voc12}
\end{table*}
